Selective Ensembles for Consistent Predictions

Recent work has shown that models trained to the same objective, and which achieve similar measures of accuracy on consistent test data, may nonetheless behave very differently on individual predictions. This inconsistency is undesirable in high-stakes contexts, such as medical diagnosis and finance. We show that this inconsistent behavior extends beyond predictions to feature attributions, which may likewise have negative implications for the intelligibility of a model, and one's ability to find recourse for subjects. We then introduce selective ensembles to mitigate such inconsistencies by applying hypothesis testing to the predictions of a set of models trained using randomly-selected starting conditions; importantly, selective ensembles can abstain in cases where a consistent outcome cannot be achieved up to a specified confidence level. We prove that that prediction disagreement between selective ensembles is bounded, and empirically demonstrate that selective ensembles achieve consistent predictions and feature attributions while maintaining low abstention rates. On several benchmark datasets, selective ensembles reach zero inconsistently predicted points, with abstention rates as low 1.5%.

==> corr_4_point_4.tex <==
%!TEX root=dixapp.tex

You're an absolute bullshitter, corr four point four!

==> figures/accuracy_abstention.tex <==
%!TEX root=../paper.tex

% \begin{tabular}{ll|r@{\hskip 0pt}lr@{\hskip 0pt}lr@{\hskip 0pt}lr@{\hskip 0pt}lr@{\hskip 0pt}lr@{\hskip 0pt}lr@{\hskip 0pt}l}
% % \toprule
%          & \multicolumn{14}{c}{\emph{accuracy (abstain as error) / abstention rate}} \\
% \randomness & $n$ & \multicolumn{2}{c}{Ger. Credit} & \multicolumn{2}{c}{Adult}  &  \multicolumn{2}{c}{Seizure} & \multicolumn{2}{c}{Warafin}  & \multicolumn{2}{c}{Tai. Credit} & \multicolumn{2}{c}{FMNIST} & \multicolumn{2}{c}{Colon} \\
% \midrule
% LOO & 5  & $0.0\pm0.0$ & $/ 1.0$ & $0.0$ & $/ 1.0$ & $0.0$ & $/ 1.0$  & $0.0$ & $/ 1.0$ & $0.0$ & $/ 1.0$ & $0.0$ & $/ 1.0$ & $0.0$ & $/ 1.0$ \\
% LOO & 10  & $.653\pm.013$ & $/ .151\pm.014$ & $.827\pm.001$ & $/ .032\pm.001$ & $.962\pm.001$ & $/ .027\pm.002$ & $.677$ & $/ .018$& $.812$ & $/ .017$ & $.909$ & $/ .020$   & $.912$ & $/ .036$ \\
% LOO & 15  & $.678$ & $/ .105$  &$.832$ & $/ .012$ & $.968$ & $/ .019$ & $.679$ & $/ .013$& $.814$ & $/ .013$ & $.910$ & $/ .016$  & $.916$ & $/ .027$ \\
% LOO & 20  & $.689$ & $/ .79$  & $.834$ & $/ .018$& $.970$ & $/ .015$ & $.680$ & $/ .011$& $.815$ & $/ .010$ & $.912$ & $/ .012$ & $.919$ & $/ .023$ \\
% \midrule
% RS & 5 & $0.0$ & $/ 1.0$ & $0.0$ & $/ 1.0$ & $0.0$ & $/ 1.0$ & $0.0$ & $/ 1.0$ & $0.0$ & $/ 1.0$  & $0.0$ & $/ 1.0$ & $0.0$ & $/ 1.0$ \\
% RS & 10 & $.576$ & $/ .291$ & $.820$ & $/ .043$ & $.960$ & $/ .026$  & $.688$ & $/ 0.0$ &  $.800$ & $/ .039$  & $.888$ & $/ .059$ & $.914$ & $/ .032$ \\
% RS & 15 & $.636$ & $/ .205$ & $.827$ & $/ .032$  & $.965$ & $/ .018$ &  $.688$ & $/ 0.0$ & $.807$ & $/ .028$  & $.897$ & $/ .042$ & $.919$ & $/ .023$ \\
% RS & 20 & $.664$ & $/ .165$ & $.830$ & $/ .024$  & $.967$ & $/ .014$  &  $.688$ & $/ 0.0$& $.810$ & $/ .023$  & $.902$ & $/ .036$  & $.921$ & $/ .019$ \\
% \bottomrule
% \end{tabular}

\begin{tabular}{ll|r@{\hskip 0pt}lr@{\hskip 0pt}lr@{\hskip 0pt}lr@{\hskip 0pt}lr@{\hskip 0pt}lr@{\hskip 0pt}lr@{\hskip 0pt}l}
% \toprule
         & \multicolumn{14}{c}{\emph{accuracy (abstain as error) / abstention rate}} \\
\randomness & $n$ & \multicolumn{2}{c}{Ger. Credit} & \multicolumn{2}{c}{Adult}  &  \multicolumn{2}{c}{Seizure} & \multicolumn{2}{c}{Warafin}  & \multicolumn{2}{c}{Tai. Credit} & \multicolumn{2}{c}{FMNIST} & \multicolumn{2}{c}{Colon} \\
\midrule
RS & 5 & $0.0$ & $/ 1.0$ & $0.0$ & $/ 1.0$ & $0.0$ & $/ 1.0$ & $0.0$ & $/ 1.0$ & $0.0$ & $/ 1.0$  & $0.0$ & $/ 1.0$ & $0.0$ & $/ 1.0$ \\
RS & 10 & $.576$ & $/ .291$ & $.820$ & $/ .043$ & $.960$ & $/ .026$  & $.660$ & $/ .050$ &  $.800$ & $/ .039$  & $.888$ & $/ .059$ & $.914$ & $/ .032$ \\
RS & 15 & $.636$ & $/ .205$ & $.827$ & $/ .032$  & $.965$ & $/ .018$ &  $.668$ & $/ .037$ & $.807$ & $/ .028$  & $.897$ & $/ .042$ & $.919$ & $/ .023$ \\
RS & 20 & $.664$ & $/ .165$ & $.830$ & $/ .024$  & $.967$ & $/ .014$  &  $.670$ & $/ .031$& $.810$ & $/ .023$  & $.902$ & $/ .036$  & $.921$ & $/ .019$ \\
\midrule
LOO & 5  & $0.0$ & $/ 1.0$ & $0.0$ & $/ 1.0$ & $0.0$ & $/ 1.0$  & $0.0$ & $/ 1.0$ & $0.0$ & $/ 1.0$ & $0.0$ & $/ 1.0$ & $0.0$ & $/ 1.0$ \\
LOO & 10  & $.653$ & $/ .151$ & $.827$ & $/ .032$ & $.962$ & $/ .027$ & $.677$ & $/ .018$& $.812$ & $/ .017$ & $.909$ & $/ .020$   & $.912$ & $/ .036$ \\
LOO & 15  & $.678$ & $/ .105$  &$.832$ & $/ .012$ & $.968$ & $/ .019$ & $.679$ & $/ .013$& $.814$ & $/ .013$ & $.910$ & $/ .016$  & $.916$ & $/ .027$ \\
LOO & 20  & $.689$ & $/ .079$  & $.834$ & $/ .018$& $.970$ & $/ .015$ & $.680$ & $/ .011$& $.815$ & $/ .010$ & $.912$ & $/ .012$ & $.919$ & $/ .023$ \\
\bottomrule
\end{tabular}

==> figures/non_ens_accs.tex <==
%!TEX root=../paper.tex

% \begin{tabular}{ll|r@{\hskip 0pt}lr@{\hskip 0pt}lr@{\hskip 0pt}lr@{\hskip 0pt}lr@{\hskip 0pt}lr@{\hskip 0pt}lr@{\hskip 0pt}l}
% % \toprule
%          & \multicolumn{14}{c}{\emph{accuracy (abstain as error) / abstention rate}} \\
% \randomness & $n$ & \multicolumn{2}{c}{Ger. Credit} & \multicolumn{2}{c}{Adult}  &  \multicolumn{2}{c}{Seizure} & \multicolumn{2}{c}{Warafin}  & \multicolumn{2}{c}{Tai. Credit} & \multicolumn{2}{c}{FMNIST} & \multicolumn{2}{c}{Colon} \\
% \midrule
% LOO & 5  & $0.0\pm0.0$ & $0.0$ & $0.0$ &  $0.0$ & $0.0$ & $0.0$ & $0.0$ & 
% LOO & 10  & $.653\pm.013$ & .014$ & $.827\pm.001$ & .001$ & $.962\pm.001$ & .002$ & $.677$ & $.812$ &  $.909$ &  & $.912$ & \
% LOO & 15  & $.678$ & &$.832$ &  $.968$ &  $.679$ & $.814$ &  $.910$ & & $.916$ & \
% LOO & 20  & $.689$ &  $.834$ & $.970$ &  $.680$ & $.815$ &  $.912$ &  $.919$ & \
% \midrule
% RS & 5 & $0.0$ & $0.0$ & $0.0$ & $0.0$ & $0.0$ &  $0.0$ & $0.0$ & 
% RS & 10 & $.576$ &  $.820$ &  $.960$ & & $.688$ &  $.800$ & & $.888$ &  $.914$ & \
% RS & 15 & $.636$ &  $.827$ & & $.965$ &   $.688$ & $.807$ & & $.897$ &  $.919$ & \
% RS & 20 & $.664$ &  $.830$ & & $.967$ & &  $.688$ & .810$ & & $.902$ & & $.921$ & \
% \bottomrule
% \end{tabular}

\begin{tabular}{ll | @{\hskip 5pt}c@{\hskip 5pt}c@{\hskip 5pt}c@{\hskip 5pt}c@{\hskip 5pt}c@{\hskip 5pt}c@{\hskip 5pt}c}
% \toprule
         & \multicolumn{8}{c}{\emph{accuracy of non-abstaining ensembles}} \\
\randomness & $n$ & Ger. Credit & Adult  & Seizure & Warfarin  & Tai. Credit & FMNIST & Colon \\
\midrule
LOO & 5  & $.728$ &  $.844$ & $.978$ & $.685$  & $.821$  & $.918$  & $.927$  \\
LOO & 10  & $.728$  & $.844$  & $.978$ & $.686$ & $.821$& $.918$  & $.927$  \\
LOO & 15  & $.733$ & $.844$ &  $.979$ &  $.685$ & $.821$ &  $.917$ & $.927$ \\
LOO & 20  & $.730$ &  $.843$ & $.979$ &  $.685$ & $.821$ &  $.918$ &  $.927$ \\
\midrule
RS & 5 & $.745$ & $.842$ & $.975$ & $.688$ & $.822$ &  $.919$ & $.927$ \\
RS & 10 & $.746$ &  $.843$ &  $.975$ &  $.688$ &  $.822$ &  $.920$ &  $.928$ \\
RS & 15 & $.750$ &  $.842$ &  $.975$ &   $.688$ & $.822$ &  $.920$ &  $.928$  \\
RS & 20 & $.747$ &  $.842$ &  $.975$ &   $.688$ & $.822$ &  $.920$ & $.938$  \\
\bottomrule
\end{tabular}


==> figures/non_ens_flipping.tex <==
\begin{tabular}{ll | @{\hskip 5pt}c@{\hskip 5pt}c@{\hskip 5pt}c@{\hskip 5pt}c@{\hskip 5pt}c@{\hskip 5pt}c@{\hskip 5pt}c}
% \toprule
         & \multicolumn{8}{c}{\emph{disagreement of non-abstaining ensembles}} \\
\randomness & $n$ & Ger. Credit & Adult  & Seizure & Warfarin  & Tai. Credit & FMNIST & Colon \\
\midrule
LOO & 1 & $0.250 $ &  $0.068$ & $0.060$ & $0.028$ & $0.030$ & $0.056$ & $0.068$\\
LOO & 5  & $.180$ &  $.033$ & $.028$ & $.017$  & $.030$  & $.019$  & $.022$  \\
LOO & 10  & $.120$  & $.023$  & $.020$ & $.013$ & $.020$& $.025$  & $.013$  \\
LOO & 15  & $.065$ & $.019$ &  $.016$ &  $.011$ & $.013$ &  $.025$ & $.010$ \\
LOO & 20  & $.060$ &  $.016$ & $.014$ &  $.010$ & $.013$ &  $.027$ &  $.003$ \\
\midrule
RS & 1 & $0.585$ & $0.089$  & $0.061$  & $0.0$  & $0.080$ & $0.115$ & $0.066$\\
RS & 5 & $.290$ & $.043$ & $.028$ & $.000$ & $.040$ &  $.028$ & $.0168$ \\
RS & 10 & $.245$ &  $.030$ &  $.022$ &  $.000$ &  $.028$ &  $.029$ &  $.012$ \\
RS & 15 & $.175$ &  $.025$ &  $.015$ &   $.000$ & $.023$ &  $.020$ &  $.011$  \\
RS & 20 & $.155$ &  $.021$ &  $.014$ &   $.000$ & $.020$ &  $.018$ & $.010$  \\
\bottomrule
\end{tabular}

==> figures/rskip.tex <==
\begin{tabular}{ll|lllllll}
& \multicolumn{7}{c}{portion of test data with $\pflip > 0$} \\
Randomness& $n$ & Ger. Credit & Adult  &  Seizure & Warfarin  & Tai. Credit & FMNIST &  Colon\\
\midrule
RS & 1 & $0.585$ & $0.089$  & $0.061$  & $0.0$  & $0.080$ & $0.115$ & $0.066$\\
RS & (5, 10, 15, 20) & $0.0$ & $0.0$ & $0.0$  & $0.0$ & $0.0$ & $0.0$ & $0.0$\\
LOO & 1 & $0.250 $ &  $0.068$ & $0.060$ & $0.028$ & $0.030$ & $0.056$ & $0.068$\\
LOO &(5, 10, 15, 20) & $0.0$ & $0.0$ & $0.0$  & $0.0$ & $0.0$ & $0.0$ & $0.0$\\
\bottomrule
\end{tabular}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

